Compact Feed-Forward 3D Gaussians via Saliency-Guided Primitive Merging

3D scene reconstruction, modeling, and rendering are highly relevant for numerous tasks, and 3D Gaussian splatting has become a standard choice in this context. Its feed-forward variants provide fast reconstruction from sparse input views but often produce per-pixel primitives, leading to highly redundant and thus inefficient representations. We present a structure-aware merging pipeline that takes per-pixel primitives from any feed-forward method and consolidates them into a compact, content-adaptive Gaussian set while largely retaining visual quality at just $\frac{1}{20}^\text{th}$ of the Gaussians of a per-pixel method. We group spatially coherent Gaussians of similar appearance into variable-size clusters via adaptive superpixel segmentation guided by a saliency map, which allocates fine segments to textured regions and coarse segments to homogeneous areas. We compress each cluster into a compact latent representation through a learned encoder, then match and consolidate representations across views based on geometric overlap and feature similarity via a learned merger. A level-of-detail decoder then produces the final Gaussians at a controllable resolution, enabling a flexible quality-efficiency trade-off at inference. As a post-processing module, the pipeline is backbone-agnostic, leveraging the strengths of existing feed-forward methods. This leads to better and more robust quality than achieved by previous approaches that target a reduction in primitive count, while providing a highly compact representation, that can be rendered efficiently.

==> pics/gen/abl_backbone_da3_posed_pareto_data.tex <==

\def\showMMval{1}
\def\hasvoxelizedval{0}
\def\hasresplatval{1}
\def\hasvolsplatval{1}

\def\paretoXmax{38}
\def\paretoXticks{5,10,15,20,30,35}
\def\paretoXlabels{5,10,15,20,93,100}
\def\breakA{0.66}
\def\breakB{0.70}

\def\pUnm{(35.00, 16.8180)}
\def\pMM{(4.87, 13.4582)}
\def\pKone{(4.41, 17.4119)}
\def\pKtwo{(8.82, 17.5369)}
\def\pKfour{(17.32, 17.5648)}
\def\pYmin{11.5}
\def\pYmax{18.5}
\def\pFront{(4.41, 17.4119) (8.82, 17.5369) (17.32, 17.5648)}

\def\sUnm{(35.00, 0.5534)}
\def\sMM{(4.87, 0.4681)}
\def\sKone{(4.41, 0.5517)}
\def\sKtwo{(8.82, 0.5551)}
\def\sKfour{(17.32, 0.5560)}
\def\sYmin{0.27}
\def\sYmax{0.6}
\def\sFront{(4.41, 0.5517) (8.82, 0.5551) (17.32, 0.5560)}

\def\lUnm{(35.00, 0.3356)}
\def\lMM{(4.87, 0.6162)}
\def\lKone{(4.41, 0.4284)}
\def\lKtwo{(8.82, 0.4253)}
\def\lKfour{(17.32, 0.4244)}
\def\lYmin{0.28}
\def\lYmax{0.7}
\def\lFront{(4.41, 0.4284) (8.82, 0.4253) (17.32, 0.4244)}

\def\pResplatInit{(6.25, 13.7017)}
\def\sResplatInit{(6.25, 0.3774)}
\def\lResplatInit{(6.25, 0.5711)}

\def\pResplat{(6.25, 15.1871)}
\def\sResplat{(6.25, 0.4408)}
\def\lResplat{(6.25, 0.5514)}

\def\pVolsplat{(30.00, 12.5437)}
\def\sVolsplat{(30.00, 0.3125)}
\def\lVolsplat{(30.00, 0.6523)}



